The discrepancy between Einstein mass and dynamical mass for SIS and power-law mass models

We investigate the discrepancy between the two-dimensional projected lensing mass and the dynam- ical mass for an ensemble of 97 strong gravitational lensing systems discovered by the Sloan Lens ACS (SLACS) Survey, the BOSS Emission-Line Lens Survey (BELLS), and the BELLS for GALaxy-Ly{\alpha} EmitteR sYs- tems (BELLS GALLERY) Survey. We fit the lensing data to obtain the Einstein mass, and use the velocity dispersion of the lensing galaxies provided by the Sloan Digital Sky Survey (SDSS) to get the projected dynamical mass within the Einstein radius by assuming the power-law mass approximation. The discrepancy is found to be obvious and quantified by Bayesian analysis. For the singular isothermal sphere (SIS) mass model, we obtain that the Einstein mass is 20.7% more than the dynamical mass, and the discrepancy increases with the redshift of the lensing galaxies. For more general power-law mass model, the discrepancy still exists within 1{\sigma} credible region. The main reason of the the discrepancy could be mass contamination, including all invisible masses along the line of sight. In addition, the measurement errors and the approximation of the mass models could lead to part of the discrepancy.

==> letter <==

We thank the referee very much for his/her advices,  we have corrected all the issues and disadvantages raised in the report as well as some other errors.

1. The main change is equation(8), we rename  s_n into s_i, and rename the \sigma_{err} into \sigma_{\rm err}^i as the referee advised. and we changes the form of equation(8), we refered to Hogg et al.(2010) to write this likelihood function  .

2. We rewrite the caption of fig5

3. We correct all the English phrasing error the referee mentioned.

4. We rewrite the first sentense in ABSTRACT








